MIRA: a Digital Signature Scheme based on the MinRank problem and the MPC-in-the-Head paradigm

We exploit the idea of [Fen22] which proposes to build an efficient signature scheme based on a zero-knowledge proof of knowledge of a solution of a MinRank instance. The scheme uses the MPCitH paradigm, which is an efficient way to build ZK proofs. We combine this idea with another idea, the hypercube technique introduced in [AMGH+22], which leads to more efficient MPCitH-based scheme. This new approach is more efficient than classical MPCitH, as it allows to reduce the number of party computation. This gives us a first scheme called MIRA-Additive. We then present an other scheme, based on low-threshold secret sharings, called MIRA-Threshold, which is a faster scheme, at the price of larger signatures. The construction of MPCitH using threshold secret sharing is detailed in [FR22]. These two constructions allows us to be faster than classical MPCitH, with a size of signature around 5.6kB with MIRA-Additive, and 8.3kB with MIRA-Threshold. We detail here the constructions and optimizations of the schemes, as well as their security proofs.

==> exec_pi_th.tex <==
\begin{figure}[H]
\pcb[codesize=\scriptsize, minlineheight=0.75\baselineskip, mode=text, width=0.98\textwidth] { 
  \textbf{Inputs:} A full set of shares $(\share{\bm{x}},\share{\bm{\beta}},\share{\bm{a}},\share{c})$ and a protocol challenge $\big( (\gamma_j)_{j \in \oneto{n}}, \epsilon \big)$\\
   \textbf{Outputs:} A set of shares $\share{v}$ and a commitment $H$ of the execution\\[\baselineskip]
  %
  For each party $i\in\oneto{N}$: \\
\pcind - Compute $\share{\bm{E}}_i = \bm{M}_0 + \sum_{j=1}^{k}[\![x_j]\!]_i\bm{M}_j$ \\ 
  \pcind - Set  $[\![e_j]\!]_i$ as the element in $\Fqm$ associated to the j-th column of $[\![E]\!]_i$ \\
  \pcind - Compute $[\![z]\!]_i = -\sum_{j=1}^n \gamma_j([\![e_j]\!]_i^{q^r})$ \\
 \pcind - For $k$ from $0$ to $r-1$: \\
\pcind  \pcind $\diamond$ Compute $[\![w_k]\!]_i=\sum_{j=1}^n \gamma_j([\![e_j]\!]_i^{q^k})$ \\
  \pcind  - Compute $[\![\bm{\alpha}]\!]_i = \epsilon \cdot [\![\bm{w}]\!]_i+[\![\bm{a}]\!]_i$ and reveal $\bm{\alpha}$ \\
  \pcind  - Compute $[\![v]\!]_i=\epsilon \cdot [\![z]\!]_i-\langle\bm{\alpha},[\![\bm{\beta}]\!]_i\rangle-[\![c]\!]_i$ \\
 The parties broadcast their shares of $\bm{\alpha}$ and $v$
  }
\vspace{-\baselineskip}
\caption{\footnotesize{Execution of the MPC protocol $\Pi^\eta$ on a full set of shares}} \label{exec_pi_th}
\end{figure}



==> fig-hvzk-thr.tex <==
%!TEX root = ./main.tex

\begin{figure}
\pcb[codesize=\scriptsize, minlineheight=0.75\baselineskip, mode=text, width=0.98\textwidth] { 
   \pcind - Public data $\bm{M}_0,\dots,\bm{M}_k \in \Fq^{m\times n}$\\ 
   [\baselineskip]
   %
  \textbf{Step 1: Sample challenges} \\
  1. The prover begin to sample challenges:\\
  \pcind \pcind - Sample the first challenge: $\ch_1=\big( (\gamma_j)_{j \in \oneto{n}}, \epsilon \big)\sampler \Fqme^n \times \Fqme$ \\
  \pcind \pcind - Sample the second challenge: $\ch_2= I \subset \oneto{N} $ of parties such that $ |I| = \ell $ \\
  [\baselineskip]
  %
  \textbf{Step 2: Compute shares and their commitments} \\
  2. The prover builds a set of shares into a $(\ell+1,N)$-threshold LSSS of a random $\bm{x'}\in\Fq^{k}$, a vector $\bm{\beta'}\in\Fqm^{r}$ which represents a random linearized polynomial and a random vector $\bm{a'}\in\Fqme^{r}$.\\
  3. The prover follows the protocol to build auxiliary values. For each party $i$ in a subset $S$:\\
  \pcind \pcind - Compute $\share{\bm{E'}}_i = \bm{M}_0 + \sum_{i=1}^{k}\bm{M}_i\share{x'}_i$ \\
  \pcind \pcind - Set $\share{e_j}_i$ as the element in $\Fqm$ associated to the j-th column of $\share{E'}$ \\
  \pcind \pcind - Compute $\share{z'}_i = - \sum\nolimits_{j = 1}^{n} \gamma_j \share{e'_j}_i^{q^r}$ \\
  \pcind \pcind -  For all $k \in [0, r - 1]$: compute $\share{w'_k}_i = \sum\nolimits_{j = 1}^{n} \gamma_j \share{e'_j}_i^{q^k}$ \\
 \pcind \pcind - Compute $\share{\boldsymbol{\alpha'}}_i = \epsilon \cdot \share{\bm{w'}}_i + \share{\bm{a'}}_i$ and reveals $\boldsymbol{\alpha'}$\\
 4. The prover chooses $c'$ such that the protocol accepts:\\
 \pcind \pcind - Compute $c'=\epsilon z' -\dotp{\boldsymbol{\alpha'}, \bm{\beta'}}$ and builds a set of shares \\
 \pcind \pcind - Compute $\share{v'}_i = \epsilon \cdot \share{z'}_i - \dotp{\boldsymbol{\alpha'}, \share{\bm{\beta'}}_i} - \share{c'}_i$ \\
 5. The prover commits the values: \\
 \pcind \pcind - Compute for each $i\in\oneto{N}$:  $\state_i=(\share{\bm{x'}}_i,\share{\bm{\beta'}}_i,\share{\bm{a'}}_i\share{c'}_i)$ and $\cmt_i=\commit{\state_i,\rho_i}$\\
 \pcind \pcind - Compute the Merkle tree root: $h_0 = \textsf{Merkle}(\cmt_1, \cdots, \cmt_N)$\\
 \pcind \pcind - Compute $h_1=\hash \left((\share{\boldsymbol{\alpha'}}_i,\share{v'}_i)_{i\in S}\right)$ \\ [\baselineskip]
 %
  \textbf{Step 3: Output transcript} \\
  6. The prover outputs the transcript $(h_0,\ch_1,\rsp_1,\ch_2,\rsp_2)$, where $\rsp_1=h_1$ and $\rsp_2=((\cmt_i)_{i\in I},\textsf{path})$, where $\textsf{path}$ is the authentication path to these commitments in the Merkle tree.
}
\vspace{-\baselineskip}
\captionof{figure}{\footnotesize{HVZK simulator of the PoK with threshold sharing}}
\label{hvzk_thr}
\MR{We don't see where the prior knowledge of $I$ is used by the simulator so there is probably an issue}
\end{figure}

==> mpc_check_hypercube.tex <==
\begin{figure}[H]
\pcb[codesize=\scriptsize, minlineheight=0.75\baselineskip, mode=text, width=0.98\textwidth] {
  \textbf{Inputs:} A leaf $i^*$ that one does not reveal, the main party shares $\share{\bm{\alpha}}$ and $\share{v}$ on which the hidden leaf $i^*$ depends on, all the other main parties shares $(\share{\bm{x}},\share{\bm{\beta}},\share{\bm{a}},\share{c})$. \\
   \textbf{Outputs:}  $\share{\bm{\alpha}},\share{v}$ and a commitment $H$ of the execution\\[\baselineskip]
  %
  \textbf{For} all the main parties:\\
  \pcind \pcind \textbf{If} the party $p$ contains the leaf $i^*$ (i.e, $p = (j,k)$ with $i^*_j = k$ as explained in Section \ref{mpc_pok}):\\
  \pcind \pcind \pcind \pcind Set $\share{v}_{i^*}$ such that $v=0$\\
  \pcind \pcind \textbf{Else}:\\
  \pcind \pcind \pcind \pcind Do the same computations as in $\Pi^\eta$ to obtain the correct shares $\share{\bm{\alpha}}_p$ and $\share{v}_p$\\
  Compute $H=\hash \left(\share{\boldsymbol{\alpha}},\share{v})\right)$
  }
\vspace{-\baselineskip}
\captionof{figure}{\footnotesize{Check the executions of the MPC protocol $\Pi^\eta$ on the main parties}}\label{check_pi_hypercube}
\end{figure}

==> mpc_exec_hypercube.tex <==
\begin{figure}[H]
\pcb[codesize=\scriptsize, minlineheight=0.75\baselineskip, mode=text, width=0.98\textwidth] { 
  \textbf{Inputs:} A full set of shares $(\share{\bm{x}},\share{\bm{\beta}},\share{\bm{a}}, \share{c})$ and a protocol challenge $\big( (\gamma_j)_{j \in \oneto{n}}, \epsilon \big)$\\
   \textbf{Outputs:} A set of shares $\share{v}$ and a commitment $H$ of the execution\\[\baselineskip]
  %
  \textbf{For} each main party $i\in\{1,2\}$: \\
\pcind - Compute $\share{\bm{E}}_i = \bm{M}_0 + \sum_{j=1}^{k}[\![x_j]\!]_i\bm{M}_j$ \\ 
  \pcind - Set  $[\![e_j]\!]_i$ as the element in $\Fqm$ associated to the j-th column of $[\![\bm{E}]\!]_i$ \\
  \pcind - Compute $[\![z]\!]_i = -\sum_{j=1}^n \gamma_j([\![e_j]\!]_i^{q^r})$ \\
 \pcind \textbf{For} $k$ from $0$ to $r-1$: \\
\pcind  \pcind $\diamond$ Compute $[\![w_k]\!]_i=\sum_{j=1}^n \gamma_j([\![e_j]\!]_i^{q^k})$ \\
  \pcind - Compute $[\![\bm{\alpha}]\!]_i = \epsilon \cdot [\![\bm{w}]\!]_i+[\![\bm{a}]\!]_i$ and reveal $\bm{\alpha}$ \\
  \pcind - Compute $[\![v]\!]_i=\epsilon \cdot [\![z]\!]_i-\langle\bm{\alpha},[\![\bm{\beta}]\!]_i\rangle-[\![c]\!]_i$ \\
 Compute: $H=\hash \left(\share{\bm{\alpha}},\share{v}\right)$
  }
\vspace{-\baselineskip}
\captionof{figure}{\footnotesize{Execution of the MPC protocol $\Pi^\eta$ on a set of main shares}}
\label{exec_pi_hypercube}
 \end{figure}
